Privacy and Customer Segmentation in the Smart Grid

In the electricity grid, networked sensors which record and transmit increasingly high-granularity data are being deployed. In such a setting, privacy concerns are a natural consideration. We present an attack model for privacy breaches, and, using results from estimation theory, derive theoretical results ensuring that an adversary will fail to infer private information with a certain probability, independent of the algorithm used. We show utility companies would benefit from less noisy, higher frequency data, as it would improve various smart grid operations such as load prediction. We provide a method to quantify how smart grid operations improve as a function of higher frequency data. In order to obtain the consumer's valuation of privacy, we design a screening mechanism consisting of a menu of contracts to the energy consumer with varying guarantees of privacy. The screening process is a means to segment customers. Finally, we design insurance contracts using the probability of a privacy breach to be offered by third-party insurance companies.

==> makefile <==
# set latexfile to the name of the main file without the .tex
latexfile = 2014arxivContracts
# put the names of figure files here.  include the .eps
#figures = 
# if no references, run "touch latexfile.bbl; touch referencefile.bib"
# or delete dependency in .dvi and tarball sections
referencefile = 2014arxivContracts

TEX = pdflatex

# support subdirectories
VPATH = Figs


# idea from http://ctan.unsw.edu.au/help/uk-tex-faq/Makefile
#$(latexfile).dvi : $(figures) $(latexfile).tex 
$(latexfile).pdf : $(figures) $(latexfile).tex $(referencefile).bbl
	while ($(TEX) $(latexfile) ; \
	grep -q "Rerun to get cross" $(latexfile).log ) do true ; \
	done


# keep .eps files in the same directory as the .fig files
#%.eps : %.fig
#	fig2dev -L eps $< > $(dir $< )$@

# The command below makes pdf from ps, call "make pdf" to run
#$(latexfile).pdf : $(latexfile).ps
#	ps2pdf $(latexfile).ps $(latexfile).pdf

#pdf : $(latexfile).pdf

# The command blow makes ps from dvi, call "make ps" to run
#$(latexfile).ps : $(latexfile).dvi
#	dvips $(latexfile)

#ps : $(latexfile).ps 

# The command below creates a tarball, call "make tarball" to run
$(latexfile).tar.gz : $(figures) $(latexfile).tex $(referencefile).bib
	tar -czvf $(latexfile).tar.gz $^

tarball: $(latexfile).tar.gz

# short cuts for multiple runs, cpall compiles all, clean removes junk, bibit runs bibtex alone
cpall:
	make; make pdf; skim $(latexfile).pdf; rm $(latexfile).dvi $(latexfile).log 
	#$(latexfile).ps
clean:
	rm $(latexfile).dvi $(latexfile).log $(latexfile).ps $(latexfile).pdf

bibit: 
	bibtex $(latexfile)

